The equivalence between many-to-one polygraphs and opetopic sets

From the polynomial approach to the definition of opetopes of Kock et al., we derive a category of opetopes, and show that its set-valued presheaves, or opetopic sets, are equivalent to many-to-one polygraphs. As an immediate corollary, we establish that opetopic sets are equivalent to multitopic sets, introduced and studied by Harnick et al, and we also address an open question of Henry.

==> macros.tex <==
\makeatletter


\newcommand{\adjunction}{
    \mathrel{\vcenter{
        \offinterlineskip\m@th
        \ialign{
            \hfil$##$\hfil\cr
            \longrightarrow\cr
            \noalign{\kern-.2ex}
            \begingroup\setlength\unitlength{.15em}
            \begin{picture} (1, 1)
                \roundcap
                \polyline (0, 0) (1, 0)
                \polyline (0.5, 0) (0.5, 1)
            \end{picture}
            \endgroup\cr
            \longleftarrow\cr
        }
    }}
}

\newcommand{\noitcnujda}{
    \mathrel{\vcenter{
        \offinterlineskip\m@th
        \ialign{
            \hfil$##$\hfil\cr
            \longleftarrow\cr
            \noalign{\kern-.2ex}
            \begingroup\setlength\unitlength{.15em}
            \begin{picture} (1, 1)
                \roundcap
                \polyline (0, 0) (1, 0)
                \polyline (0.5, 0) (0.5, 1)
            \end{picture}
            \endgroup\cr
            \longrightarrow\cr
        }
    }}
}

\newcommand{\longadjunction}{
    \mathrel{\vcenter{
        \offinterlineskip\m@th
        \ialign{
            \hfil$##$\hfil\cr
            \relbar\joinrel\relbar\joinrel\relbar\joinrel\relbar\joinrel\relbar\joinrel\rightarrow\cr
            \noalign{\kern-.2ex}
            \begingroup\setlength\unitlength{.15em}
            \begin{picture} (1, 1)
                \roundcap
                \polyline (0, 0) (1, 0)
                \polyline (0.5, 0) (0.5, 1)
            \end{picture}
            \endgroup\cr
            \leftarrow\joinrel\relbar\joinrel\relbar\joinrel\relbar\joinrel\relbar\joinrel\relbar\cr
        }
    }}
}

\newcommand{\longhookrightarrow}{
    \mathrel{
        \hookrightarrow
        \!\!\!\!
        \tikz \fill[white] (0, 0) rectangle (.1,.4);
        \!\!\!\!\!\!
        \relbar
        \!\!
        \rightarrow
    }
}

\newcommand{\longleadsto}{
        \begin{tikzcd} [ampersand replacement = \&]
            ~
                \ar[r, rightsquigarrow] \&
            ~
        \end{tikzcd}
    }

\newcommand*{\xto}[1]{\xrightarrow{\substack{\hphantom{\quad}\\{#1}}}}
\newcommand*{\xot}[1]{\xleftarrow{\substack{\hphantom{\quad}\\{#1}}}}
\newcommand{\wedgearrow}{\xto{\cdot\,\cdot}}



\renewcommand{\op}{\mathrm{op}}

\newcategory{\Cart}{}{C}{art}
\newcategory{\Ctx}{}{C}{tx}

\newcategory{\psh}{}{P}{sh}

\newcommand{\Psh}[1]{\psh (#1)}
\newcommand{\PshO}{{\Psh\bbOO}}


\DeclareMathOperator{\eqdef}{\mathbin{\coloneq}}
\DeclareMathOperator{\equivdef}{\mathbin{:\!\equiv}}
\newcommand{\hash}{\#}
\DeclareMathOperator{\Lan}{Lan}
\DeclareMathOperator{\Ran}{Ran}
\newcommand{\condition}[1]{\textbf{\upshape{(#1)}}}
\newcommand{\qqquad}{\qquad\qquad}

\newcommand{\spcong}{\:\cong\:}
\newcommand{\speq}{\:=\:}
\newcommand{\speqdef}{\:\eqdef\:}

\DeclareMathOperator{\shriek}{!}

\theoremstyle{definition}
\newtheorem{assumption}[axiom]{Assumption}
\newtheorem{assumptions}[axiom]{Assumptions}
\crefname{assumption}{assumption}{assumptions}


\newcommand{\optPolyFun}{\frakZZ}
\newcommand{\opetope}[1]{\left\lbrace\begin{matrix*}[l]#1\end{matrix*}\right.}
\newcommand{\degenopetope}[1]{\left\lbrace \!\! \opetope{#1} \right.}
\newcommand{\sep}{\leftarrow}

\newcommand{\optZero}{\filledlozenge}
\newcommand{\optOne}{\filledsquare}
\newcommand{\optInt}[1]{\mathbf{#1}}

\newcommand{\shape}[1]{#1^\natural}
\newcommand{\universal}{\filledtriangleright}


\DeclareMathOperator{\ct}{ct}
\newcategory{\Pol}{}{P}{ol}
\newcommand{\composition}[1]{#1^\circ}
\newcommand{\ctxplace}{\Box}
\newcommand{\MTO}{\mathrm{mto}}
\newcommand{\PolMTO}{\Pol^\MTO}
\newcommand{\polyreal}[1]{\vert #1 \vert}
\newcommand{\Oplex}{\bbOO\mathrm{plex}}


\DeclareMathOperator{\elt}{elt}
\newcategory{\PolyEnd}{}{P}{oly{\catEE}nd}
\newcategory{\PolyMnd}{}{P}{oly{\catMM}nd}
\newcategory{\Tree}{}{T}{ree}
\newcommand{\elTree}{\Tree_{\mathrm{elem}}}

\newcommand{\polynomialfunctor}[7]{
    \begin{tikzcd}
        [ampersand replacement = \&]
        \displaystyle{#1}       \&
        \displaystyle{#2}
            \ar[l, "#5" above]
            \ar[r, "#6" above]  \&
        \displaystyle{#3}
            \ar[r, "#7" above]  \&
        \displaystyle{#4}
    \end{tikzcd}
}
\newcommand{\polynomialinline}[4]{
    #1 \longleftarrow #2 \longrightarrow #3 \longrightarrow #4
}


\newcommand{\DDownarrow}{
    \mathrel{
        \begin{tikz} [baseline=-3pt, rotate=-90]
            \draw [shorten >= 0pt, shorten <= 0pt]
                (0, 3pt)  -- ++(1.5ex, 0)
                (0, 1pt)  -- ++(1.5ex+1pt, 0)
                (0, -1pt) -- ++(1.5ex + 1pt, 0)
                (0, -3pt) -- ++(1.5ex, 0)
                (1.5ex - 1pt, 5pt)
                    to [in = 135, out = -75] (1.5ex + 2pt, 0)
                    to [out = -135, in = 75] (1.5ex - 1pt, -5pt);
        \end{tikz}
    }
}

\newcommand{\RRightarrow}{
    \mathrel{
        \begin{tikz} [baseline=-3pt]
            \draw [shorten >= 0pt, shorten <= 0pt]
                (-3pt, 3pt) -- (0, 3pt)  -- ++(1.5ex,0)
                (-3pt, 1pt) -- (0, 1pt)  -- ++(1.5ex+1pt, 0)
                (-3pt, -1pt) -- (0, -1pt) -- ++(1.5ex + 1pt, 0)
                (-3pt, -3pt) -- (0, -3pt) -- ++(1.5ex, 0)
                (1.5ex - 1pt, 5pt)
                    to [in = 135, out = -75] (1.5ex + 2pt, 0)
                    to [out = -135, in = 75] (1.5ex - 1pt, -5pt);
        \end{tikz}
    }
}

\newcommand{\tikzinput}[3][1]{
    \begin{tikzpicture}
        \tikzset{scale = #1}
        \ExecuteMetaData[tikz/#2.tikz]{main}
        \@for\tmp:=#3\do{
            \ExecuteMetaData[tikz/#2.tikz]{\tmp}
        }
    \end{tikzpicture}
}

\renewcommand{\ulcorner}{\lefthalfcap}
\renewcommand{\lrcorner}{\righthalfcup}
\newcommand{\pullbackcorner}{
    \ar[dr, phantom, "\lrcorner", very near start, shift right = 0ex]
}
\newcommand{\pushoutcorner}{
    \ar[dr, phantom, "\ulcorner", very near end, shift right = 0ex]
}


\newcommand{\itree}[1]{\mathsf{I}_{#1}}
\newcommand{\ytree}[1]{\mathsf{Y}_{#1}}

\newcommand{\edgesymbol}{\medvert}  %
\newcommand{\leafsymbol}{\medvert}  %
\newcommand{\nodesymbol}{\bullet}

\DeclareMathOperator{\tree}{tr}
\DeclareMathOperator{\treewithleaf}{tr^{\leafsymbol}}
\DeclareMathOperator{\treewithnode}{tr^{\nodesymbol}}

\newcommand{\underlyingtree}[1]{\langle #1 \rangle}

\DeclareMathOperator{\addr}{\&}

\newcommand{\subst}{\operatornamewithlimits{\smallsquare}}
\newcommand{\graft}{\operatornamewithlimits{\circ}}
\newcommand{\grafti}{\operatornamewithlimits{\tilde{\circ}}}
\DeclareMathOperator*{\biggraft}{\bigcircle}
\DeclareBigOperator{\bigsubst}{\Box}

\DeclareMathOperator{\barsrc}{\overline{\src}}
\DeclareMathOperator{\edg}{\mathsf{e}}
\DeclareMathOperator{\src}{\mathsf{s}}
\DeclareMathOperator{\tgt}{\mathsf{t}}
\DeclareMathOperator{\var}{\mathsf{v}}

\DeclareMathOperator{\mndr}{\rho}
\DeclareMathOperator{\readdress}{\wp}
\newcommand{\mndop}{\operatornamewithlimits{\wedge}}
\newcommand{\bigmndop}{\bigwedge}

\makeatother


==> tikz/common.tex <==
\input{tikz-config.tex}

% args: x, y, w, h, label, inner x, innner y
\newenvironment{TIKZZONE}[7]{
    \begin{scope} [shift = {(#1, #2)}]
        \draw [dotted] (0, 0) node [above right]
            {\small{\texttt{#5}}} -- (0, #4) -- (#3, #4) -- (#3, 0) -- cycle;
        \begin{scope} [shift = {(#6, #7)}]
}{
        \end{scope}
    \end{scope}
}

\newcommand{\blackwhitespoon}{-}
\newcommand{\DDownarrow}{|}
\newcommand{\optInt}[1]{\textbf{#1}}
\newcommand{\optOne}{\rightarrow}
\newcommand{\optZero}{\bullet}
\newcommand{\readdress}{P}
\newcommand{\RRightarrow}{-}
\newcommand{\Rrightarrow}{\equiv\!>}
\newcommand{\shape}[1]{{#1}^\natural}
\newcommand{\smalltriangleright}{>}
\newcommand{\src}{\mathsf{s}}
\newcommand{\system}{\textsc}
\newcommand{\tgt}{\mathsf{t}}

==> tikz/tikz-config.tex <==
\usetikzlibrary{
    backgrounds,
    calc,
    cd,
    decorations.pathmorphing,
    patterns,
    positioning,
    shapes,
}

\tikzset{baseline = (current bounding box.center)}

\tikzset{aCircle/.style = {
    circle,
    minimum size = 7pt,
    inner sep = 0,
    draw,
    fill = green
}}

\tikzset{aDiamond/.style = {
    diamond,
    minimum size = 7pt,
    inner sep = 0,
    draw,
    fill = blue
}}

\tikzset{aPentagon/.style = {
    regular polygon,
    minimum size = 7pt,
    inner sep = 0,
    draw,
    fill = red
}}

\tikzset{aStar/.style = {
    star,
    star points = 7,
    minimum size = 7pt,
    inner sep = 0,
    draw,
    fill = yellow
}}

\tikzset{treeedge/.style = {above, sloped}}

\tikzset{treenode/.style = {
    circle, minimum size = 2pt, inner sep = 0, draw, fill
}}

\tikzset{bigtreenode/.style = {
    circle, minimum size = 4pt, inner sep = 0, draw, fill
}}

\newcommand{\partnodetext}[2]{\tiny{Part \ref{#1}: #2}}
\newcommand{\chapternodetext}[2]{
    \tiny{Chapter \ref{#1}}
    \nodepart{second}
    {\small{#2}}
}
\newcommand{\vplaceholder}{\\ ~ \phantom{for opetopes}}
